FutureMapping 2: Gaussian Belief Propagation for Spatial AI

We argue the case for Gaussian Belief Propagation (GBP) as a strong algorithmic framework for the distributed, generic and incremental probabilistic estimation we need in Spatial AI as we aim at high performance smart robots and devices which operate within the constraints of real products. Processor hardware is changing rapidly, and GBP has the right character to take advantage of highly distributed processing and storage while estimating global quantities, as well as great flexibility. We present a detailed tutorial on GBP, relating to the standard factor graph formulation used in robotics and computer vision, and give several simulation examples with code which demonstrate its properties.

==> newcom.tex <==
% Content of newcom.tex was merged with symbols.tex.
% 
% You do not need to include this file anymore. This file is here only to ensure 
% backwards compatibility.
 

